Score Change of Variables

We derive a general change of variables formula for score functions, showing that for a smooth, invertible transformation $\mathbf{y} = \phi(\mathbf{x})$, the transformed score function $\nabla_{\mathbf{y}} \log q(\mathbf{y})$ can be expressed directly in terms of $\nabla_{\mathbf{x}} \log p(\mathbf{x})$. Using this result, we develop two applications: First, we establish a reverse-time It\^o lemma for score-based diffusion models, allowing the use of $\nabla_{\mathbf{x}} \log p_t(\mathbf{x})$ to reverse an SDE in the transformed space without directly learning $\nabla_{\mathbf{y}} \log q_t(\mathbf{y})$. This approach enables training diffusion models in one space but sampling in another, effectively decoupling the forward and reverse processes. Second, we introduce generalized sliced score matching, extending traditional sliced score matching from linear projections to arbitrary smooth transformations. This provides greater flexibility in high-dimensional density estimation. We demonstrate these theoretical advances through applications to diffusion on the probability simplex and empirically compare our generalized score matching approach against traditional sliced score matching methods.

==> Condtional_Score_Cov.tex <==
\section{Conditional Scores and the Change of Variables}

\subsection{Conditional Scores}

For a joint distribution $p(\mathbf{x}, \mathbf{y})$, the conditional score of $\mathbf{x}$ given $\mathbf{y}$ is:

\begin{equation}
\nabla_{\mathbf{x}} \log p(\mathbf{x} | \mathbf{y}) = \nabla_{\mathbf{x}} \log p(\mathbf{x}, \mathbf{y}) - \nabla_{\mathbf{x}} \log p(\mathbf{y})
\end{equation}

This follows from the chain rule: $p(\mathbf{x}, \mathbf{y}) = p(\mathbf{x} | \mathbf{y}) p(\mathbf{y})$.

\subsection{Transformation}

Consider a smooth, invertible transformation:

\begin{align}
\mathbf{u} &= \phi(\mathbf{x}, \mathbf{y}) \\
\mathbf{v} &= \psi(\mathbf{x}, \mathbf{y})
\end{align}

We want to find $\nabla_{\mathbf{u}} \log q(\mathbf{u} | \mathbf{v})$, where $q$ is the joint density in the transformed space.

\subsection{Applying the Score Change of Variables Formula}

We apply the score change of variables formula (Theorem 1) to both the joint score $\nabla_{\mathbf{x},\mathbf{y}} \log p(\mathbf{x}, \mathbf{y})$ and the marginal score $\nabla_{\mathbf{x}} \log p(\mathbf{y})$.

\subsubsection{Transforming the Joint Score}

Let $\mathbf{J}$ be the Jacobian of the inverse transformation from $(\mathbf{u}, \mathbf{v})$ to $(\mathbf{x}, \mathbf{y})$. Applying the formula to $\nabla_{\mathbf{x},\mathbf{y}} \log p(\mathbf{x}, \mathbf{y})$ gives an expression involving:

\begin{itemize}
    \item $\mathbf{J}^\top$
    \item $\nabla_{\mathbf{x},\mathbf{y}} \log p(\mathbf{x}, \mathbf{y})$
    \item $\nabla_{\mathbf{x},\mathbf{y}} \cdot \left( \mathbf{J}^\top \right)$
\end{itemize}

We then take the part of the result corresponding to the gradient with respect to $\mathbf{u}$.

\subsubsection{Transforming the Marginal Score}

We treat $p(\mathbf{y})$ as a function of $\mathbf{x}$ and apply the formula to $\nabla_{\mathbf{x}} \log p(\mathbf{y})$. This involves a different Jacobian, say $\mathbf{J}_m$, because we are only concerned with the variation of $p(\mathbf{y})$ as $\mathbf{x}$ changes. This gives an expression involving:
\begin{itemize}
    \item $\mathbf{J}_m^\top$
    \item $\nabla_{\mathbf{x}} \log p(\mathbf{y})$
    \item $\nabla_{\mathbf{x}} \cdot \left( \mathbf{J}_m^\top \right)$
\end{itemize}
We take the part of the result corresponding to the gradient with respect to $\mathbf{u}$.

\subsection{The Interaction}

The transformed conditional score $\nabla_{\mathbf{u}} \log q(\mathbf{u} | \mathbf{v})$ is the difference of the transformed joint and marginal scores. Importantly, the Jacobian and divergence terms **do not generally cancel out** because $\mathbf{J}$ and $\mathbf{J}_m$ are different. The transformation of the marginal score does not have a simple general form.

\subsection{Implications}

\begin{itemize}
    \item Transforming conditional scores is complex due to the interaction between the transformation and conditioning.
    \item Special cases (e.g., factorized transformations, specific transformation families) might lead to simplifications.
    \item Potential applications in conditional score-based models and inference in transformed spaces.
\end{itemize}
